Beyond Online Balanced Descent: An Optimal Algorithm for Smoothed Online Optimization

We study online convex optimization in a setting where the learner seeks to minimize the sum of a per-round hitting cost and a movement cost which is incurred when changing decisions between rounds. We prove a new lower bound on the competitive ratio of any online algorithm in the setting where the costs are $m$-strongly convex and the movement costs are the squared $\ell_2$ norm. This lower bound shows that no algorithm can achieve a competitive ratio that is $o(m^{-1/2})$ as $m$ tends to zero. No existing algorithms have competitive ratios matching this bound, and we show that the state-of-the-art algorithm, Online Balanced Decent (OBD), has a competitive ratio that is $\Omega(m^{-2/3})$. We additionally propose two new algorithms, Greedy OBD (G-OBD) and Regularized OBD (R-OBD) and prove that both algorithms have an $O(m^{-1/2})$ competitive ratio. The result for G-OBD holds when the hitting costs are quasiconvex and the movement costs are the squared $\ell_2$ norm, while the result for R-OBD holds when the hitting costs are $m$-strongly convex and the movement costs are Bregman Divergences. Further, we show that R-OBD simultaneously achieves constant, dimension-free competitive ratio and sublinear regret when hitting costs are strongly convex.

==> Acknowledgements.tex <==
Gautam Goel, Yiheng Lin, and Haoyuan Sun contributed equally to this work. Gautam Goel was supported by an Amazon AI Fellowship. Adam Wierman was supported by grants AitF-1637598 and CNS-1518941.


==> Discussion.tex <==

\begin{comment}

In this section, we compare G-OBD and R-OBD on their generality, performance bound, and information need.

We first compare the generality. As for hitting cost functions, G-OBD can work for quasi-convex hitting cost functions (Theorem \ref{OBD_PLUS_T1}), while the competitive ratio we proved for R-OBD (Theorems \ref{thm-Breg-cr}) only holds for strongly convex hitting cost functions. On the other hand, Theorem \ref{thm-Breg-cr} shows R-OBD can work for Bregman Divergence switching costs with respect to general norms, while G-OBD only works for $\ell_2$ quadratic switching costs. Since $\ell_2$ quadratic is a special case of Bregman Divergence, R-OBD are more general when it comes to switching costs and general norms.

Then we compare the performance. Although the competitive ratio of G-OBD is bounded by constant times the optimal competitive ratio (Theorem \ref{OBD_PLUS_T1}), the competitive ratio of R-OBD matches exactly with the general lower bound (Theorem \ref{thm-optimal-cr} and Theorem \ref{GeneralLowerT1}). So we conclude that R-OBD performs much better than G-OBD.

Finally, we compare the information used by G-OBD and R-OBD. It is clear that R-OBD uses much less information than G-OBD because all we need to do in R-OBD is searching the minimizer of a strongly convex function, while G-OBD requires doing projections onto different level sets for multiple times.

In conclusion, the choice of algorithms should be made in an ad hoc way. Although we have enumerate more advantages of R-OBD than G-OBD, there are still some specific problems which require the use of G-OBD.


\end{comment}









\begin{comment}
\subsection{Tendency towards the Minimizer: Similarity among examples}
\input{Main_Similarity.tex}

\subsection{Trade-off: Information VS. Generality}
\input{Main_Tradeoff.tex}

\subsection{Example Applications for Bregman Divergence Switching Cost}
\input{Main_Example.tex}
\end{comment}

==> Figure_OBDLowerProof1.tex <==
\begin{figure}[h!]
\begin{center}
\begin{asy}
size(10cm);
defaultpen(fontsize(6pt));

real sq = sqrt(10);

pair A = (1, 6);
pair B = (1, 1);
pair C = (16, 1);
pair D = (1 + 4.5*sq, 6 - 1.5*sq);

pair E = (1, 1.5);
pair F = (1.5, 1.5);
pair G = (1.5, 1);

pair H = (1 + 0.5*sq, 1 - 1.5*sq);
pair I = (1 + 5*sq, 1);

pair ArcStart = (1 + 0.5*sq, 6 + 1.5*sq);
pair ArcEnd = (16 + 5*sq, 6);

pair H2 = (4 + 0.5*sq, -3 - 1.5*sq);
pair I2 = (16 + 0.5*sq, 6 - 1.5*sq);

pair X = (20, 1);
pair Y = (16, 5);

pair O = (8.5+2.5*sq, 3.5);
real R1 = 2.5*sqrt(20 - 6*sq);
real R2 = 2.5*sqrt(20 + 6*sq);

dot(A, red+linewidth(3));
label("$x_{t-1}$", A, N);
dot(B, red+linewidth(3));
label("$x_t$", B, S);
dot(C, red+linewidth(3));
label("$x_t^*$", C, S);
dot(D, red+linewidth(3));
label("$x_{t-1}^*$", D, N);
dot(H, red+linewidth(3));
label("$x_{t+1}$", H, S);
dot(I, red+linewidth(3));
label("$x_{t+1}^*$", (17.5, 1), S);
dot(O, red+linewidth(3));
label("$O$", O, N);

dot(H2, red+linewidth(3));
label("$x_{t+2}$", H2, S);
dot(I2, red+linewidth(3));
label("$x_{t+2}^*$", I2, N);

//label("$x$", X, S);
//label("$y$", Y, W);

label("$h$", (1, 3.5), W);
label("$h$", (1.75, -1.37), W);
label("$\ell$", (8.1, 3.6), N);
label("$\ell$", (8.5, 1), N);
label("$\ell$", (9.7, -1.37), N);

draw(A--B, blue);
draw(B--C, blue);
draw(A--C, blue);
draw(B--H, dashed+blue);
draw(H--I, dashed+blue);
draw(H--H2, dashed+blue);
draw(I--I2, dashed+blue);
draw(H2--I2, dashed+blue);

//draw(E--F, blue);
//draw(F--G, blue);

//draw(C--X, EndArrow);
//draw(C--Y, EndArrow);

pen circlePen=green+1bp+opacity(0.8);

draw(circle(O, R1), circlePen);
draw(arc(O, A, ArcEnd), circlePen);
\end{asy}
\end{center}
\caption{Counterexample used in Theorem \ref{OBDLowerT1}.In the figure, $x_{t-1}, x_t, \cdots, x_{t+2}$ represent the sequence of points picked by OBD, $x_{t-1}^*, x_t^*, \cdots, x_{t+2}^*$ represent the sequence of points picked by the offline adversary. \adam{we don't need to repeat the figure, just refer to the earlier one.}}
\label{figure:OBDLowerProof1}
\end{figure}

==> Main_Example.tex <==
Section 3.3 of \cite{chen2018smoothed} gives three mirror maps that are commenly used for OMD. All of them are both strongly convex and strongly smooth with respect to some norm $\norm{\cdot}$. Thus they can be used as the potential h for Bregman Divergence Switching cost.

\subsubsection{Euclidean norm squared}
$h(x) = \frac{1}{2}\norm{x}_2^2$ are both 1-strongly convex and 1-strongly smooth with respect to L2 norm.

\subsubsection{Mahalanobis distance square}
When Q is positive definite, $h(x) = \frac{1}{2}\norm{x}_Q^2$ is 1-strongly convex and 1-strongly smooth with respect to Mahalanobis distance $\norm{\cdot}_Q$.

\subsubsection{Negative Entropy}
In the simplex
$$X = P_\delta = \{x | \sum_{i=1}^n x_i = 1, x_i \geq \delta\}$$
the negative entropy function $h(x) = \sum_{i=1}^n x_i \ln x_i$ is $\frac{1}{2\ln 2}-$strongly convex and $\frac{1}{\delta \ln 2}-$strongly smooth.

==> Main_RG.tex <==
As for Regularized Greedy Algorithm, we can prove that even when the cost functions are not m-strongly convex, we can still achieve a constant optimal competitive ratio.

\begin{theorem}\label{thm-RG-CR}
If the potential function $h(x)$ is $\alpha-$strongly convex and $\beta-$strongly smooth with respect to some norm $\norm{\cdot}$, and the cost function $f_t(x)$ is convex and satisfies that $\forall x, f_t(x) \geq \frac{m}{2}\norm{x - v_t}^2$. Then Regularized Greedy with some parameter $\lambda$ can achieve a competitive ratio of $1 + \frac{\beta}{\sqrt{\alpha m}}$.
\end{theorem}

Actually, we can prove a more general bound for the competitive ratio which is a function of $\lambda$.

\begin{theorem}\label{RG_CR_T1}
If the potential function $h(x)$ is $\alpha-$strongly convex and $\beta-$strongly smooth with respect to some norm $\norm{\cdot}$, and the cost function $f_t(x)$ is convex and satisfies that $\forall x, f_t(x) \geq \frac{m}{2}\norm{x - v_t}^2$.
Then Regularized Greedy with parameter $\lambda > 0$ can achieve a competitive ratio of
$$\max \{1 + \frac{\lambda \beta}{m}, 1 + \frac{\beta}{\lambda \alpha}\}$$
\end{theorem}

Solving the equation $1 + \frac{\lambda \beta}{m} = 1 + \frac{\beta}{\lambda \alpha}$, we get $\lambda = \sqrt{\frac{m}{\alpha}}$, which promises a competitive ratio of
$1 + \frac{\beta}{\sqrt{\alpha m}}$ as stated in Theorem \ref{thm-RG-CR}.

==> Main_Similarity.tex <==
Surprisingly, all examples with good competitive ratio of the new algorithm shows a tendency to move towards the minimizer. Among them, the Regularized Greedy is the most obvious one, because it can be interpreted as step-wise Greedy plus a regularizer towards $v_t$.

$$x_t = \argmin_x \big( C_t(x) + D_h(x || x_{t-1})\big) + \lambda_2 D_h(x || v_t)$$

Although Weighted Greedy looks very different from Regularized Greedy and $v_t$ is absent from its expression, if we rewrite it in the form:

$$x_t = \argmin_x C_t(x) + \lambda_1 D_h(x || x_{t-1}) = \argmin_x \big(C_t(x) + D_h(x || x_{t-1})\big) + \frac{1 - \lambda_1}{\lambda_1} C_t(x)$$

The term $\frac{1 - \lambda_1}{\lambda_1} C_t(x)$ serves almost the same as the previous regularizer $\lambda_2 D_h(x || v_t)$. When $C_t(x) = \frac{m}{2}\norm{x - v_t}_2^2$ and $h(x) = \frac{1}{2}\norm{x}_2^2$, to achieve the optimal competitive ratio, we have
$$\frac{1 - \lambda_1}{\lambda_1} = \frac{1}{2}( - 1 + \sqrt{1 + \frac{4}{m}})$$
$$\lambda_2 = \frac{m}{2}( - 1 + \sqrt{1 + \frac{4}{m}})$$
Thus the two regularizers are exactly the same! (i.e. $\frac{1 - \lambda_1}{\lambda_1}C_t(x) = \lambda_2 D_h(x||v_t)$) However, this also suggests that when the shape of the cost function is very different from L2 quadratic, the performance of Weighted Greedy and Regularized Greedy can be different.

==> Main_Tradeoff.tex <==
Among all the algorithms we proposed, OBD PLUS uses the largest amount of information about the hitting cost function (Doing projection on different level sets); Weighted Greedy uses the smallest (Only need to query gradients at several points); Regularized Greedy lies in the middle (It need gradients and the location of $v_t$). Does the increment of information improve the ability for generalization?

Theorem \ref{WG_tradeT1} suggests that OBD+ can do much better than Weighted Greedy when the hitting cost functions are quasi-convex. 

\begin{theorem}\label{WG_tradeT1}
When the constraints for the hitting cost functions are $f_t(x) - f_t(v_t) \geq \frac{m}{2}\norm{x - v_t}_2^2$ and $f_t(x)$ is quasi-convex, and the moving cost is $M(x_t, x_{t-1}) = \frac{1}{2}\norm{x_t - x_{t-1}}_2^2$, the competitive ratio of Weighted Greedy is at least $\Omega(\frac{1}{m})$.
\end{theorem}

Under the common constraint that the hitting cost functions are $f_t(x) - f_t(v_t) \geq \frac{m}{2}\norm{x - v_t}_2^2$, and the moving cost is $M(x_t, x_{t-1}) = \frac{1}{2}\norm{x_t - x_{t-1}}_2^2$, we collect the facts we present before:
\begin{enumerate}
    \item OBD+ can achieve a $O(\sqrt{\frac{1}{m}})$ competitive ratio when hitting costs are quasi-convex;
    \item Regularized Greedy can achieve a $O(\sqrt{\frac{1}{m}})$ competitive ratio when hitting costs are convex; \textcolor{purple}{Yiheng: Actually, the result is even stronger.}
    \item Weighted Greedy can achieve a $O(\sqrt{\frac{1}{m}})$ competitive ratio when hitting costs are m-strongly convex;
    \item The competitive ratio of Weighted Greedy is at least $\Omega(\frac{1}{m})$ when hitting costs are quasi-convex.
\end{enumerate}

Based on these results, we conjecture that the ability of generalization increases as the information increases.

\textcolor{purple}{Yiheng: Without the convex assumption (for example, quasi-convex), can we prove a $O(\frac{1}{m})$ competitive ratio for Regularized Greedy? Just like GREEDY algorithm.}

\begin{comment}
Suppose Weighted Greedy is minimizing the following function in L2 case:
$$H(x) = C_t(x) + \lambda_1\cdot \frac{1}{2}\norm{x - x_{t-1}}_2^2$$
Suppose the starting point is $x_0 = 0$. We can construct a function $f: \mathbb{R} \to \mathbb{R}$, which satisfies that:
\begin{enumerate}
    \item f is quasi-convex and $f(x) \geq \frac{m}{2}(x - v)^2$ for some $m > 0, v > 0$;
    \item $\argmin_x f(x) + \frac{\lambda_1}{2}x^2 = 0$.
\end{enumerate}
\begin{center}
\begin{tikzpicture}
      \draw[->] (-2,0) -- (2,0) node[right] {$x$};
      \draw[->] (0,-1) -- (0,2) node[above] {$f(x)$};
      \draw[scale=0.5,domain=-1:0,smooth,variable=\x,blue]  plot ({\x},{(\x - 1)*(\x - 1)});
      \draw[scale=0.5,domain=0:1,smooth,variable=\x,blue] plot ({\x},{1 - \x*\x});
      \draw[scale=0.5,domain=1:3,smooth,variable=\x,blue]  plot ({\x},{(\x - 1)*(\x - 1)});
\end{tikzpicture}
\end{center}
In the game, we propose $C_t(x) = f(x), t = 1, 2, \cdots$.

Since we always have $\argmin_x H(x) = 0 = x_0$, Weighted Greedy will not move at all. So the competitive ratio becomes unbounded.

However, both OBD Plus and Regularized Greedy still have bounded competitive ratio in this case.

OBD or OBD PLUS is immune to this example, because they can promise the claimed CR for quasi-convex hitting functions.

For Regularized Greedy, at least it will move towards the minimizer at each step step. And we have
$$|x_t - v| \leq \frac{\lambda_2}{\lambda_1 + \lambda_2}|x_{t-1} - v|$$
So the competitive ratio is bounded.

Actually, for any quasi-convex hitting cost functions, the competitive ratio of Regularized Greedy will be bounded. Since only when the offline stays at $v_{t_0}$ and does not move at all time steps $t \geq t_0$ , the competitive ratio can tend to $\infty$. But with the knowledge of minimizer, Regularized Greedy always moves towards $v_{t_0}$.
\end{comment}

==> NewOutline.tex <==
\subsection*{2. Model and Preliminaries}
\subsubsection*{2.1 Model}
\subsubsection*{2.2 OBD}
\subsection*{3. Lower Bounds}
\subsubsection*{3.1 General Lower Bound}
Theorem \ref{GeneralLowerT1}.
\subsubsection*{3.2 OBD Lower Bound}
Lemma \ref{OBDLowerL1} and Theorem \ref{OBDLowerT1}.
\subsection*{4. Improving OBD}
\subsubsection*{Greedy OBD}
(which is called OBD Plus in the draft)

Section 4.1 in this draft. Theorem \ref{OBD_PLUS_T1}.
\subsubsection*{Regularized OBD}
(which is called Triple Terms in the draft)

"Local" view of MD/OBD?

Section 5 in this draft. Theorem \ref{MainT0}, \ref{MainT1}, \ref{RG_CR_T1} in this order.
\subsubsection*{Discussion}
Compare bounds and generality and simplicity of new algorithms.

Please refer to Section 5.4 in this draft.
\subsection*{Regret VS. Competitive ratio}

Theorem \ref{WGRegretT1}.
\subsection*{Conclusion}

==> RG_CR_T1.tex <==
\textcolor{blue}{Fixed. Ready for reviewing.}
\begin{proof}[Proof of Theorem \ref{RG_CR_T1}]
Notice that since $f_t(x) + D_h(x || x_{t-1}) + \lambda D_h(x || v_t)$ is strongly convex and differentiable, we can restate the update rule as
$$\nabla f_t(x_t) = \left( \nabla h(x_{t-1}) - \nabla h(x_t)\right) + \lambda \left( \nabla h(v_t) - \nabla h(x_t)\right).$$

Notice that $h$ is $\alpha-$strongly convex and $\beta-$strongly smooth with respect to norm $\norm{\cdot}$. Thus we can give a trivial upper and lower bound of Bregman Divergence, which is
\begin{equation}\label{RG_CR_T1_E0}
    \forall x, y, \frac{\alpha}{2}\norm{x - y}^2 \leq D_h(x || y) \leq \frac{\beta}{2}\norm{x - y}^2.
\end{equation}

Since $f_t(x)$ is convex, we further obtain
\begin{equation}\label{RG_CR_T1_E1}
    \begin{aligned}
    f_t(x_t^*) &\geq f_t(x_t) + \langle \nabla f_t(x_t), x_t^* - x_t\rangle\\
    &= f_t(x_t) - \langle \nabla h(x_{t-1}) - \nabla h(x_t), x_t - x_t^* \rangle - \lambda \langle \nabla h(v_t) - \nabla h(x_t), x_t - x_t^* \rangle.
    \end{aligned}
\end{equation}
Using lemma \ref{GWGL1}, we notice that
\begin{equation}\label{RG_CR_T1_E2}
    \langle \nabla h(x_{t-1}) - \nabla h(x_t), x_t - x_t^* \rangle = \left(D_h(x_t^* || x_{t-1}) - D_h(x_t^* || x_t)\right) - D_h(x_t || x_{t-1}),
\end{equation}
and
\begin{equation}\label{RG_CR_T1_E3}
    \langle \nabla h(v_t) - \nabla h(x_t), x_t - x_t^* \rangle = \left(D_h(x_t^* || v_t) - D_h(x_t^* || x_t)\right) - D_h(x_t || v_t).
\end{equation}
Taking \ref{RG_CR_T1_E2} and \ref{RG_CR_T1_E3} into inequality \ref{RG_CR_T1_E1}, we obtain
$$f_t(x_t) + D_h(x_t || x_{t-1}) + \lambda D_h(x_t || v_t) + (1 + \lambda)D_h(x_t^* || x_t)\leq f_t(x_t^*) + D_h(x_t^* || x_{t-1}) + \lambda D_h(x_t^* || v_t).$$
Throwing away the term $\lambda D_h(x_t || v_t)$ from the left hand side, we get
$$f_t(x_t) + D_h(x_t || x_{t-1}) + (1 + \lambda)D_h(x_t^* || x_t)\leq f_t(x_t^*) + D_h(x_t^* || x_{t-1}) + \lambda D_h(x_t^* || v_t).$$
Define the potential function as $\phi(x_t, x_t^*) = (1 + \lambda) D_h(x_t^* || x_t)$. For convenience, we define $\Delta \phi = \phi(x_t, x_t^*) - \phi(x_{t-1}, x_{t-1}^*)$. Using this notation, we obtain
\begin{equation}\label{RG_CR_T1_E4}
    H_t + M_t + \Delta \phi \leq \left(H_t^* + \lambda D_h(x_t^* || v_t)\right) + D_h(x_t^* || x_{t-1}) - (1 + \lambda) D_h(x_{t-1}^* || x_{t-1}).
\end{equation}
We further notice that
\begin{equation}\label{RG_CR_T1_E5}
    \begin{aligned}
    &D_h(x_t^* || x_{t-1}) - (1 + \lambda) D_h(x_{t-1}^* || x_{t-1})\\
    =&\left(D_h(x_t^* || x_{t-1}) - D_h(x_{t-1}^* || x_{t-1})\right) - \lambda D_h(x_{t-1}^* || x_{t-1})\\
    =& D_h(x_t^* || x_{t-1}^*) + \langle \nabla h(x_{t-1}) - \nabla h(x_{t-1}^*), x_{t-1}^* - x_t^* \rangle - \lambda D_h(x_{t-1}^* || x_{t-1})\\
    \leq& D_h(x_t^* || x_{t-1}^*) + \norm{\nabla h(x_{t-1}) - \nabla h(x_{t-1}^*)}_* \norm{x_{t-1}^* - x_t^*} - \lambda D_h(x_{t-1}^* || x_{t-1})\\
    \leq& D_h(x_t^* || x_{t-1}^*) + \frac{\lambda}{2\beta}\norm{\nabla h(x_{t-1}) - \nabla h(x_{t-1}^*)}_*^2 +  \frac{\beta}{2\lambda}\norm{x_{t-1}^* - x_t^*}^2  - \lambda D_h(x_{t-1}^* || x_{t-1})\\
    \leq& D_h(x_t^* || x_{t-1}^*) + \frac{\beta}{2\lambda}\norm{x_{t-1}^* - x_t^*}^2\\
    \leq& \left(1 + \frac{\beta}{\lambda \alpha}\right)D_h(x_t^* || x_{t-1}^*),
    \end{aligned}
\end{equation}
where we use general Cauchy-Schwarz in the first inequality; AM-GM in the second inequality; \ref{RG_CR_T1_E0} in the penultimate and the last inequalities.

By combining \ref{RG_CR_T1_E4} and \ref{RG_CR_T1_E5}, we obtain
\begin{equation}\label{RG_CR_T1_E6}
    H_t + M_t + \Delta \phi \leq \big(H_t^* + \lambda D_h(x_t^* || v_t)\big) + (1 + \frac{\beta}{\lambda \alpha})M_t^*.
\end{equation}
And using \ref{RG_CR_T1_E0} and the condition that $f_t$ is m-strongly convex, we see
\begin{equation}\label{RG_CR_T1_E7}
    \begin{aligned}
    \lambda D_h(x_t^* || v_t) \leq \frac{\lambda\beta}{2}\norm{x_t^* - v_t}^2\leq \frac{\lambda\beta}{m}H_t^*.
    \end{aligned}
\end{equation}
Combining \ref{RG_CR_T1_E6} and \ref{RG_CR_T1_E7}, we obtain
$$H_t + M_t + \Delta \phi \leq (1 + \frac{\lambda\beta}{m})H_t^* + (1 + \frac{\beta}{\lambda \alpha})M_t^*.$$
\end{proof}

==> WGRegretT1.tex <==
\begin{proof}[Proof of Theorem \ref{WGRegretT1}]
In the proof, we use a similar framework as the proof of Theorem 10 in \cite{chen2018smoothed}. The roughy idea is to first give an upper bound on the difference of hitting costs ($f_t(x_t) - f_t(x_t^L)$), then prove a sub linear upper bound for $\sum_{t=1}^T \left(f_t(x_t) - f_t(x_t^L) + M(x_t, x_{t-1}) \right)$.

Since function $f_t(x) + \lambda D_h(x || x_{t-1})$ is strongly convex, we can restate the update as
$$\nabla f_t(x) = \lambda \left( \nabla h(x_{t-1}) - \nabla h(x_t)\right).$$

Therefore by Lemma \ref{GWGL1}, we have
\begin{equation*}
    \begin{aligned}
    \langle \nabla f_t(x_t), x_t - x_t^L \rangle &= \lambda \langle \nabla h(x_{t-1}) - \nabla h(x_t), x_t - x_t^L \rangle\\
    &= \lambda \left(D_h(x_t^L || x_{t-1}) - D_h(x_t^L || x_t)\right) - \lambda D_h(x_t || x_{t-1}).
    \end{aligned}
\end{equation*}
Thus for some parameter $q > 0$ which we will define later, we obtain
\begin{equation}\label{GWGRegret1}
    \begin{aligned}
    & f_t(x_t) - f_t(x_t^L) \\
    \leq& \langle \nabla f_t(x_t), x_t - x_t^L \rangle - \frac{m}{2}\norm{x_t - x_t^L}^2\\
    =& \lambda \left(D_h(x_t^L || x_{t-1}) - D_h(x_t^L || x_t)\right) - \lambda D_h(x_t || x_{t-1}) - \frac{m}{2}\norm{x_t - x_t^L}^2\\
    =& (\lambda + q) \left(D_h(x_t^L || x_{t-1}) - D_h(x_t^L || x_t)\right) - \lambda D_h(x_t || x_{t-1})\\ 
    &- \left(q D_h(x_t^L || x_{t-1}) - q D_h(x_t^L || x_t) + \frac{m}{2}\norm{x_t - x_t^L}^2\right).\\
    \end{aligned}
\end{equation}
Using lemma \ref{GWGL1}, we obtain
\begin{equation}\label{GWGRegretE2}
    \begin{aligned}
    &q D_h(x_t^L || x_{t-1}) - q D_h(x_t^L || x_t) + \frac{m}{2}\norm{x_t - x_t^L}^2\\
    =& q D_h(x_t || x_{t-1}) + q\langle \nabla h(x_{t-1}) - \nabla h(x_t), x_t - x_t^L\rangle + \frac{m}{2}\norm{x_t - x_t^L}^2\\
    \geq& q D_h(x_t || x_{t-1}) - q\norm{\nabla h(x_{t-1}) - \nabla h(x_t)}_* \norm{x_t - x_t^L} + \frac{m}{2}\norm{x_t - x_t^L}^2\\
    \geq& q D_h(x_t || x_{t-1}) - \big(\frac{q^2}{2m}\norm{\nabla h(x_{t-1}) - \nabla h(x_t)}_*^2 + \frac{m}{2}\norm{x_t - x_t^L}^2\big) + \frac{m}{2}\norm{x_t - x_t^L}^2\\
    =& q D_h(x_t || x_{t-1}) - \frac{q^2}{2m}\norm{\nabla h(x_{t-1}) - \nabla h(x_t)}_*^2\\
    \geq& q D_h(x_t || x_{t-1}) - \frac{\beta q^2}{m}D_h(x_t || x_{t-1})\\
    \geq& (q - \frac{\beta q^2}{m})D_h(x_t || x_{t-1}),
    \end{aligned}
\end{equation}
where we use AM-GM inequality on line 4;$\beta-$smoothness of $h$ and Theorem \ref{DualNormT1} on line 6.

In order to maximize the coefficient $(q - \frac{\beta q^2}{m})$, we fix $q = \frac{m}{2\beta}$. By taking \ref{GWGRegretE2} back to \ref{GWGRegret1}, we obtain
\begin{equation}\label{GWGRegretE3}
    f_t(x_t) - f_t(x_t^L) \leq (\lambda + \frac{m}{2\beta}) \Big(D_h(x_t^L || x_{t-1}) - D_h(x_t^L || x_t)\Big) - (\lambda + \frac{m}{4\beta}) D_h(x_t || x_{t-1}).
\end{equation}
Using the condition that $\lambda + \frac{m}{4\beta} \geq 1$, we see
\begin{equation}\label{GWGRegretE4}
    f_t(x_t) - f_t(x_t^L) + D_h(x_t || x_{t-1}) \leq (\lambda + \frac{m}{2\beta}) \Big(D_h(x_t^L || x_{t-1}) - D_h(x_t^L || x_t)\Big).
\end{equation}
We also notice that
\begin{equation}\label{GWGRegretE5}
    \sum_{t=1}^T \norm{x_t^L - x_{t+1}^L} \leq \sqrt{T\left( \sum_{t=1}^T \norm{x_t^L - x_{t+1}^L}^2 \right)} \leq \sqrt{T\left( \sum_{t=1}^T \frac{2D_h(x_{t+1}^L || D_h(x_t^L))}{\alpha} \right)} \leq \sqrt{\frac{2TL}{\alpha}}.
\end{equation}
By lemma \ref{GWGL2}, we can give an upper bound of the sum of the right hand side term of \ref{GWGRegretE4}:
\begin{equation}\label{GWGRegretE6}
    \begin{aligned}
    &\sum_{t=1}^T D_h(x_t^L || x_{t-1}) - D_h(x_t^L || x_t)\\
    =& \sum_{t=1}^T \left( D_h(0 || x_{t-1}) - D_h(0 || x_t) + \langle \nabla h(x_t) - \nabla h(x_{t-1}), x_t^L\rangle \right)\\
    =& D_h(0 || x_0) - D_h(0 || x_T) + \sum_{t=1}^{T-1}\langle \nabla h(x_t), x_t^L - x_{t+1}^L\rangle - \langle \nabla h(x_0), x_1^L\rangle + \langle \nabla h(x_T), x_T^L\rangle\\
    =& \sum_{t=1}^T \langle \nabla h(x_t), x_t^L - x_{t+1}^L \rangle \\
    \leq& \sum_{t=1}^T \norm{\nabla h(x_t)}_* \norm{x_t^L - x_{t+1}^L} \\
    \leq& G\sum_{t=1}^T \norm{x_t^L - x_{t+1}^L}\\
    \leq& G\sqrt{\frac{2TL}{\alpha}},
    \end{aligned}
\end{equation}
where in line 4 we use the fact that $x_0 = x_0^L = x_{T+1}^L = 0, \nabla h(0) = 0$; in line 5 we use general Cauchy-Schwarz inequality; in the last inequality we use \ref{GWGRegretE5}.

Therefore we obtain
\begin{equation}
    \begin{aligned}
    &cost(OBD) - cost(OPT(L))\\
    =& \sum_{t=1}^T\left(f_t(x_t) - f_t(x_t^L)\right) + \sum_{t=1}^T \left(D_h(x_t || x_{t-1}) - D_h(x_t^L || x_{t-1}^L)\right)\\
    \leq& \sum_{t=1}^T\left(f_t(x_t) - f_t(x_t^L) + D_h(x_t || x_{t-1})\right) - L\\
    \leq& (\lambda + \frac{m}{2\beta})G\sqrt{\frac{2TL}{\alpha}} - L,
    \end{aligned}
\end{equation}
where we use the definition of $cost(OPT(L))$ in the first inequality; \ref{GWGRegretE4} and \ref{GWGRegretE6} in the second inequality.
\end{proof}
